Leveraging Multi-Instance GPUs through moldable task scheduling

NVIDIA MIG (Multi-Instance GPU) allows partitioning a physical GPU into multiple logical instances with fully-isolated resources, which can be dynamically reconfigured. This work highlights the untapped potential of MIG through moldable task scheduling with dynamic reconfigurations. Specifically, we propose a makespan minimization problem for multi-task execution under MIG constraints. Our profiling shows that assuming monotonicity in task work with respect to resources is not viable, as is usual in multicore scheduling. Relying on a state-of-the-art proposal that does not require such an assumption, we present FAR, a 3-phase algorithm to solve the problem. Phase 1 of FAR builds on a classical task moldability method, phase 2 combines Longest Processing Time First and List Scheduling with a novel repartitioning tree heuristic tailored to MIG constraints, and phase 3 employs local search via task moves and swaps. FAR schedules tasks in batches offline, concatenating their schedules on the fly in an improved way that favors resource reuse. Excluding reconfiguration costs, the List Scheduling proof shows an approximation factor of 7/4 on the NVIDIA A30 model. We adapt the technique to the particular constraints of an NVIDIA A100/H100 to obtain an approximation factor of 2. Including the reconfiguration cost, our real-world experiments reveal a makespan with respect to the optimum no worse than 1.22x for a well-known suite of benchmarks, and 1.10x for synthetic inputs inspired by real kernels. We obtain good experimental results for each batch of tasks, but also in the concatenation of batches, with large improvements over the state-of-the-art and proposals without GPU reconfiguration. Beyond the algorithm, the paper demonstrates the research potential of the MIG technology and suggests useful metrics, workload characterizations and evaluation techniques for future work in this field.

==> pseudocode/repartitioning_method.tex <==
\newcommand\mycommfont[1]{\fontsize{8.5}{8.5} \ttfamily\textcolor{blue!70!}{#1}}
\SetCommentSty{mycommfont}

%\begin{center}

\begin{algorithm}[t!]
 \caption{Non-moldable instance scheduling by repartition}\label{alg:repartitioning_method}

\DontPrintSemicolon
  \KwData{Set of instance sizes $C_G$, task times $t_{i=1} ^n$ and an allotment $a^k$}
  \KwResult{List $schedule$ with the begin time and slices used by each task}

$schedule := \lbrack\,\rbrack$ \tcp{Init empty schedule}
  
  \tcp{Hashmap of instance sizes to task times according to the allotment:}

  $s\_task := \big\{ s: \big\lbrack \{index:i,\, time: t_i(s)\}\;|\; a^k_i = s,\,1 \leq i \leq n \big\rbrack,\,s \in C_G\big\}$
  
    \tcp{Sort the tasks of each instance size by decreasing time:}
  sort($s\_task\lbrack s\rbrack$, sort\_key = $task \rightarrow task.time$) for each $s \in C_G$


\tcp{Define order of instances according to the completion time:}

  $less := (inst_1, inst_2) \rightarrow inst_1.b + inst_1.t < inst_2.b + inst_2.t$

\tcp{Min heap with a non-task instance $(t = 0)$ with all slices $[0, \max(C_G)]$:}

$pq$ := PQ\big(\big\lbrack $\text{Inst}(b = 0,\,t = 0,\, ls = 0,\, rs = \max(C_G))$\big\rbrack, sort\_key = $less$\big)


\While(\tcp*[h]{While there are unscheduled tasks}){$s\_times$ is not empty }{
    $last := pq$.pop() \tcp{Get first finished instance}
    \If(\tcp*[h]{If the instance is a task}){$last.t > 0$}{
        $schedule.\text{append}(last)$ \tcp{Add task to the schedule}
    }

    $size := (last.ls + 1 - last.rs)$ \tcp{Get size from boundary slices}
    
    $next\_b := last.b + last.t$ \tcp{Begin next right after}

    \tcp{Tasks of $size$ slices or $size=4$ and unscheduled 3-size tasks:}
    \If{$size \in s\_times$ or $(size = 4 \text{ and } 3 \in s\_times)$}{
         $use\_size := size \textbf{ if } size \in s\_times \textbf{ else } 3$
         
         $next := last\lbrack use\_size\rbrack.\text{pop\_front}()$ \tcp{Largest task of $use\_size$}
        
        $pq$.push\big($\text{Inst}(b = next\_b,\, t = next.time,\, ls = last.ls,$
        $rs = last.rs, \, i = next.index)\big)$ \tcp{Add the task to the heap}
    
    }
    \ElseIf(\tcp*[h]{If no task of instance size $> 1$}){$last.rs > last.rl$}{

        $lm = last.rl + (size + 1) / 2$ \tcp{Middle slice of the instance}
        \tcp{Add sub-instances to the heap;}
        $pq$.push\big($\text{Inst}(b=next\_b,\, t = 0,\, ls = last.ls,\, lr = lm-1)\big)$
    
        $pq$.push\big($\text{Inst}(b=next\_b,\, t = 0,\, ls = lm,\, lr = last.lr)\big)$

        
    }

}

\tcp{Save in $schedule$ the last scheduled tasks that are still in $pq$}

\end{algorithm}
%%\vspace{-25pt}

%\end{center}

